Online Continual Learning Via Candidates Voting

Continual learning in online scenario aims to learn a sequence of new tasks from data stream using each data only once for training, which is more realistic than in offline mode assuming data from new task are all available. However, this problem is still under-explored for the challenging class-incremental setting in which the model classifies all classes seen so far during inference. Particularly, performance struggles with increased number of tasks or additional classes to learn for each task. In addition, most existing methods require storing original data as exemplars for knowledge replay, which may not be feasible for certain applications with limited memory budget or privacy concerns. In this work, we introduce an effective and memory-efficient method for online continual learning under class-incremental setting through candidates selection from each learned task together with prior incorporation using stored feature embeddings instead of original data as exemplars. Our proposed method implemented for image classification task achieves the best results under different benchmark datasets for online continual learning including CIFAR-10, CIFAR-100 and CORE-50 while requiring much less memory resource compared with existing works.

==> method_existing.tex <==
% online results for CIFAR-100 -------------------------------------------
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/online_10.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/online_20.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(b)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/online_50.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(c)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/online_100.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(d)}
\end{minipage}
\begin{center}
\vspace{-.9cm}
\caption{\textbf{Results on Split CIFAR-100} by comparing with existing online methods with different exemplar size. The accuracy is measured after learning of each task on all tasks seen so far. (Best viewed in color)}
\label{fig: online result on cifar}
\end{center}
% \vspace{-.3cm}
\end{figure*}





% table for online results ----------------------------------
\begin{table*}[t]
    \vspace{-0.3cm}
    \centering
    \scalebox{1.}{
    \begin{tabular}{ccccccccc}
        \hline
        Datasets & \multicolumn{8}{c}{\textbf{Split CIFAR-100}}  \\
        \hline
        Size of exemplar set & \multicolumn{2}{c}{$K = 1,000$} & \multicolumn{2}{c}{$K = 2,000$} & \multicolumn{2}{c}{$K = 5,000$} & \multicolumn{2}{c}{$K = 10,000$}\\
        \hline
        Accuracy(\%) & Avg & Last & Avg & Last & Avg & Last & Avg & Last \\
        \hline
        \hline
        A-GEM~\cite{A-GEM}  & 13.9 & 4.3 & 14.1& 4.83& 13.8 & 4.4 & 13.9 & 4.5 \\
        MIR~\cite{aljundi_mir} & 37.4 & 19.1& 41.9 & 26.1 & 44.4 & 27.9 & 46.3 & 34.0 \\
        GSS~\cite{NEURIPS2019_e562cd9c_GSS} & 24.2 & 12.9 & 26.9 & 16.7 & 31.5 & 23.1 & 43.2 & 23.3 \\
        ASER~\cite{shim2020online_ASER} & 29.9 & 21.6 & 40.9 & 27.8 & 41.2 &29.5 & 43.3 & 30.8\\
        GDUMB~\cite{prabhu2020gdumb_online} & 38.3 & 20.7 & 39.2 & 26.4 & 43.8 & 31.6 & 52.8 & 39.2\\
        \hline
        Ours (without EA) & 48.4 & 32.1& 50.4& 34.5& 53.6 & \textbf{38.1} & 54.1 & \textbf{40.4}\\
        Ours & \textbf{50.6} & \textbf{35.9} & \textbf{52.0} & \textbf{36.7} & \textbf{54.2} & 37.5 & \textbf{54.9} & 40.3 \\
        \hline
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Average accuracy and Last step accuracy on Split CIFAR-100}. Best results marked in bold.  }
    \label{tab:online_cifar}
\end{table*}




%table for offline results -------------------------------
\begin{table*}[t]
    \vspace{-0.3cm}
    \centering
    \scalebox{1.}{
    \begin{tabular}{ccccccccc|cc|cc}
        \hline
        Datasets & \multicolumn{8}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{|c}{\textbf{ImageNet-100}} & \multicolumn{2}{|c}{\textbf{ImageNet-1000}}\\
        \hline
        Step size& \multicolumn{2}{c}{5} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{50} & \multicolumn{2}{|c}{10} & \multicolumn{2}{|c}{100}\\
        \hline
        Accuracy(\%) & Avg & Last & Avg & Last & Avg & Last & Avg & Last & Avg & Last & Avg & Last\\
        \hline
        \hline
        LWF~\cite{LWF}  & 29.7 & 15.5 & 39.7 & 24.0 & 47.1 &35.1 & 52.6 & 52.6& 60.7 & 36.6 & 56.5 & 39.0\\
        ICARL~\cite{ICARL} & 59.7 & 46.0 & 61.6& 51.0 & 63.3 & 56.5 & 60.7 & 60.7 & 81.8 & 63.8 & 63.7 & 44.0\\
        EEIL~\cite{EEIL} & 63.4 & 48.0 & 63.6& 51.5 & 64.2 & 57.1 & 61.2 & 61.2& 89.2 & 80.2 & 72.2 & 52.0 \\
        BIC~\cite{BIC} & 62.1 & 48.2& 63.5&52.0 & 65.1 &58.5  & 64.9 & 64.9 & 89.8 & 84.4 & 82.9 & 73.2\\
        WA~\cite{mainatining} & 62.6 & 49.6& 64.5& 53.5& 66.6 & 59.2 & 65.1 & 65.1 & 90.2 & 84.1 & \textbf{85.7} & \textbf{81.1}\\
        \hline
        Ours  & \textbf{70.6} & \textbf{57.0} & \textbf{69.9}&\textbf{59.3} & \textbf{70.5} & \textbf{62.4 }&\textbf{65.7} & \textbf{65.7} & \textbf{92.4} & \textbf{87.2} & 72.7 & 62.7 \\
        \hline
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Average accuracy and Last step accuracy on CIFAR-100 and ImageNet}. Note that the compared methods are implemented in offline while ours is implemented in online. The detail results for each learning step can be found in supplementary material. Best results marked in bold. }
    \label{tab:offline_all3}
\end{table*}

% ablation study figures---------
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.31\linewidth}
    \centering
    \includegraphics[width=5cm,height=4.5cm]{exp_new/ablation_cifar.png}
    \parbox{15.5cm}{\small \hspace{3.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.31\linewidth}
    \centering
    \includegraphics[width=5cm,height=4.5cm]{exp_new/ablation_img100.png}
    \parbox{15.5cm}{\small \hspace{3.cm}(b)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.31\linewidth}
    \centering
    \includegraphics[width=5cm,height=4.5cm]{exp_new/ablation_img1000.png}
    \parbox{15.5cm}{\small \hspace{3.cm}(c)}
\end{minipage}
\begin{center}
\vspace{-.7cm}
\caption{\textbf{Ablation study} (a) results on CIFAR-100 with step size 10 (b) results on ImageNet-100 with step size 10 (c) results on ImageNet-1000 with step size 100. (Best viewed in color)}
\vspace{-.2cm}
\label{fig:ablation}
\end{center}
\end{figure*}

% ablation study confusion matrix
\begin{figure*}[t!]
\vspace{-0.2cm}
\centering
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=5cm,height=4.5cm]{exp_new/con_1.png}
    %\parbox{15.5cm}{\small \hspace{3.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=5cm,height=4.5cm]{exp_new/con_2.png}
    %\parbox{15.5cm}{\small \hspace{3.cm}(b)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=6cm,height=4.5cm]{exp_new/con_3.png}
    %\parbox{15.5cm}{\small \hspace{3.cm}(c)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=6cm,height=4.5cm]{exp_new/con_4.png}
    %\parbox{15.5cm}{\small \hspace{3.cm}(c)}
\end{minipage}
\begin{center}
\vspace{-.5cm}
  \caption{\textbf{Confusion matrices on CIFAR-100} with step size 10 of different approaches. (Best viewed in color)}
  \vspace{-.7cm}
%\vspace{-1.1cm}
\label{fig:confusion}
\end{center}
\end{figure*}


% bias norm comparision 

\begin{figure}[t]
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/norms_new1.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/norms_new2.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(b)}
\end{minipage}
\begin{center}  %\vspace{-0.2cm}
%   \caption{\textbf{Norms of the weight vectors on CIFAR-100} with step size 10 of different approaches. The line is obtained by using linear least square to show the trend for each method. Note that we remove the first step as inapplicable for incremental learning. (Best viewed in color)}
%   \vspace{-.7cm}
  \label{fig:weightnorm}
\end{center}
\end{figure}

==> oldexp.tex <==
% table ---------------------------------------------------------
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/cifar_5.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/cifar_10.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(b)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/cifar_20.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(c)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/cifar_50.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(d)}
\end{minipage}
\begin{center}
\vspace{-.8cm}
\caption{\textbf{Results on CIFAR-100} by comparing with offline approaches with step size (a) 5, (b) 10, (c) 20 and (d) 50. Note that only our method is implemented in online. (Best viewed in color)}
\label{fig:offlinecifar}
\end{center}
% \vspace{-.3cm}
\end{figure*}


\begin{table*}[t!]
    % \vspace{-0.3cm}
    \centering
    \scalebox{1.}{
    \begin{tabular}{ccccccccc|cc|cc}
        \hline
        Datasets & \multicolumn{8}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{|c}{\textbf{ImageNet-100}} & \multicolumn{2}{|c}{\textbf{ImageNet-1000}}\\
        \hline
        Step size& \multicolumn{2}{c}{5} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{50} & \multicolumn{2}{|c}{10} & \multicolumn{2}{|c}{100}\\
        \hline
        Accuracy(\%) & Avg & Last & Avg & Last & Avg & Last & Avg & Last & Avg & Last & Avg & Last\\
        \hline
        \hline
        LWF~\cite{LWF}  & 29.7 & 15.5 & 39.7 & 24.0 & 47.1 &35.1 & 52.6 & 52.6& 60.7 & 36.6 & 56.5 & 39.0\\
        ICARL~\cite{ICARL} & 59.7 & 46.0 & 61.6& 51.0 & 63.3 & 56.5 & 60.7 & 60.7 & 81.8 & 63.8 & 63.7 & 44.0\\
        EEIL~\cite{EEIL} & 63.4 & 48.0 & 63.6& 51.5 & 64.2 & 57.1 & 61.2 & 61.2& 89.2 & 80.2 & 72.2 & 52.0 \\
        BIC~\cite{BIC} & 62.1 & 48.2& 63.5&52.0 & 65.1 &58.5  & 64.9 & 64.9 & 89.8 & 84.4 & 82.9 & 73.2\\
        WA~\cite{mainatining} & 62.6 & 49.6& 64.5& 53.5& 66.6 & 59.2 & 65.1 & 65.1 & 90.2 & 84.1 & \textbf{85.7} & \textbf{81.1}\\
        \hline
        Ours  & \textbf{70.6} & \textbf{57.0} & \textbf{69.9}&\textbf{59.3} & \textbf{70.5} & \textbf{62.4 }&\textbf{65.7} & \textbf{65.7} & \textbf{92.4} & \textbf{87.2} & 72.7 & 62.7 \\
        \hline
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Average accuracy and Last step accuracy on CIFAR-100 and ImageNet}. Note that the compared methods are implemented in offline while ours is implemented in online. Best results marked in bold. }
    \label{tab:offline_all3}
\end{table*}

% ----------------------------------------------------------------------
\section{Experimental Results}
\label{experimental results}
The structure of the experiment part is illustrated as following. 

In this section, we first compare our method with existing \textit{replay-based} online approaches including A-GEM~\cite{A-GEM}, GSS~\cite{NEURIPS2019_e562cd9c_GSS},  MIR~\cite{aljundi_mir}, ASER~\cite{shim2020online_ASER} and GDUMB~\cite{prabhu2020gdumb_online} following experiment setting similar in~\cite{GEM,A-GEM}. Then we show the effectiveness of our method by comparing with state-of-the-art offline approaches as well including LWF~\cite{LWF}, ICARL~\cite{ICARL}, EEIL~\cite{EEIL}, BIC~\cite{BIC} and WA~\cite{mainatining} by following the protocol suggested in~\cite{ICARL}. Finally we conduct further experiments to analyze the weight bias problem as well as comparing the memory storage consumption with existing methods, which will be illustrated in Section~\ref{}   



The proposed online continual learning method under class-incremental setting is compared with both the state-of-the-art \textit{online methods} following experiment setting similar in~\cite{GEM,A-GEM}, and \textit{offline continual learning methods} under benchmark protocol~\cite{ICARL}, which are illustrated in Section~\ref{exp:compare with online} and Section~\ref{exp:compare with offline}, respectively. Finally, we study the weight bias problem in online scenario and analyze the storage consumption in Section~\ref{exp:Analysis of Weights Bias, Memory}. We ran each experiment five times and report the average results.




\subsection{Datasets}
\label{exp:compare with online}
We compare our method with existing \textit{replay-based} online approaches including A-GEM~\cite{A-GEM}, GSS~\cite{NEURIPS2019_e562cd9c_GSS},  MIR~\cite{aljundi_mir}, ASER~\cite{shim2020online_ASER} and GDUMB~\cite{prabhu2020gdumb_online}. The objective is to learn a sequence of new tasks from a data stream in online scenario.

\textbf{Dataset: }We use Split CIFAR-100~\cite{zenke2017continual_splitcifar} for evaluation, which contains 20 tasks with non-overlapping classes constructed using CIFAR-100~\cite{CIFAR}. Each task contains 2,500 training images and 500 test images corresponding to 5 classes and no task index is provided during inference. 

\textbf{Model: }A small version of ResNet-18 (reduced ResNet-18)~\cite{GEM} pretrained on ImageNet~\cite{IMAGENET1000} is applied as the backbone model for all the methods. The ResNet implementation follows the setting as suggested in~\cite{RESNET}. 

\textbf{Implementation detail: }The network is trained using SGD optimizer with a mini-batch size of 10 and a fixed learning rate of 0.1. We vary the size of exemplar set for $Q \in \{1,000, 2,000, 5,000, 10,000\}$ for comparisons. 


% \subsection{Evaluation Metrics}
% \label{subsec:metrics}

\subsection{Implementation Details}
\label{subsec:metrics}

\subsection{Results on CIFAR-10 and CIFAR-100}
\label{expres:splitcifar}
Figure~\ref{fig: online result on cifar} shows the results for continual learning of 20 tasks in online scenario on Split CIFAR-100. The model is evaluated after learning of each task on test data belonging to all classes seen far. Given different exemplar size $Q$, our method is able to outperform the existing online approaches especially by a larger margin when $Q$ is smaller, \textit{i.e. }our method performs better even with limited storage capacity. The reason is that our method is not solely relied on exemplars to retain old knowledge but maintain the classifier's discriminability for each learned task and make the prediction through candidates selection and prior incorporation. We then analyze the impact of exemplar augmentation (EA) in our method as described in Section~\ref{method: learning phase}. Table~\ref{tab:online_cifar} summarizes the average accuracy (Avg) and last step accuracy (Last) for all methods, where Avg is obtained by averaging all the accuracy obtained after learning each task, which shows the overall performance for the entire continual learning procedure. We observe that our method still achieves better results even without the augmentation step. In addition, our EA is shown to be more effective to earn additional performance gains when the stored exemplar is not sufficient. Note that although increasing the number of stored exemplar is an effective strategy to improve performance for most replay based methods such as GDUMB~\cite{prabhu2020gdumb_online}, the storage capacity is a significant constrain for continual learning especially in online scenario. 



% ablation study figures----------------------------------------------------
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/ablation_cifar.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/ablation_cifar20.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(b)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/ablation_img100.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(c)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.22\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/ablation_img1000.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(d)}
\end{minipage}
\begin{center}
\vspace{-.7cm}
\caption{\textbf{Ablation study} (a) results on CIFAR-100 with step size 10 (b) results on CIFAR-100 with step size 20 (c) results on ImageNet-100 with step size 10 (d) results on ImageNet-1000 with step size 100. (Best viewed in color)}
\vspace{-.2cm}
\label{fig:ablation}
\end{center}

\end{figure*}
%------------------------------------------------------------------------

% ablation study confusion matrix------------------------------------

\begin{figure*}[t!]
\vspace{-0.3cm}
\begin{center}
  \includegraphics[width=1.\linewidth]{exp_new/confusion.pdf}
  \caption{\textbf{Confusion matrices on CIFAR-100} with step size 10 of different approaches. (Best viewed in color)}
  \vspace{-.5cm}
  \label{fig:confusion }
\end{center}
\end{figure*}


%------------------------------------------------------------------------

% \subsection{Compare With Offline Methods}
% \label{exp:compare with offline}
% In this part, we compare our proposed method implemented in online scenario with offline continual learning methods including LWF~\cite{LWF}, ICARL~\cite{ICARL}, EEIL~\cite{EEIL}, BIC~\cite{BIC} and WA~\cite{mainatining}. We follow the proposed benchmark protocol~\cite{ICARL} for class-incremental learning and the objective is to learn new classes while maintaining performance on all classes seen so far.  

% \textbf{Datasets: }We use CIFAR-100~\cite{CIFAR} and ImageNet~\cite{IMAGENET1000} and vary the learning step size for evaluation. For CIFAR-100, we divided it into splits of 5, 10, 20, and 50 classes, resulting in 20, 10, 5, and 2 learning steps respectively. There are two settings for ImageNet including (1) ImageNet-1000 containing 1000 classes with splits of 100 classes and (2) ImageNet-100 containing a subset of 100 randomly selected classes with splits of 10 classes per step. Top-1 accuracy is used for CIFAR-100 and Top-5 accuracy is reported for ImageNet. Note that the class-incremental learning starts from the second learning step under this protocol. 

% \textbf{Model: }For experiments on CIFAR-100, we apply ResNet-50 pretrained on ImageNet as feature extractor in our method with the extracted feature of dimension $2,048$. For ImageNet, we apply the ResNet-18 pretrained on Places-205~\cite{places-205}, which is a large scale dataset containing 205 scene categories and 2.5 millions annotated images. We also provide the experimental results for pretrained model on Food-101~\cite{Food-101} in the supplementary material. 

% \textbf{Implementation detail: }We apply SGD optimization with mini-batch size of 10 and a fixed learning rate of 0.1 for our method implemented in online scenario. The detail settings for all compared offline methods can be found in supplementary material. For all the experiments, we arrange classes using identical random seed~\cite{ICARL} and use fixed size of exemplar set as $Q= 2,000$ for CIFAR-100, ImageNet-100 and $Q= 20,000$ for ImageNet-1000. 
% \vspace{-0.1cm}
% \subsubsection{Results on CIFAR-100 and ImageNet}
% \label{exp:offlinecifarimagenet}
% \vspace{-0.1cm}
% We implement our proposed method in online scenario to use each data only once for training while all the compared existing methods are implemented in offline. The results on CIFAR-100 for each incremental step are shown in Figure~\ref{fig:offlinecifar}. In addition, Table~\ref{tab:offline_all3} summarizes the results for average accuracy (Avg) and Last step accuracy (Last). Our method achieves better results for all incremental step sizes on CIFAR-100, particularly for smaller step size, where the weight bias problem becomes more severe in offline case as the number of incremental steps increased.  This is alleviated significantly in online scenario, which will be analyzed in detail later in Section~\ref{exp:Analysis of Weights Bias, Memory}. The results on ImageNet-100 also show positive improvement using our method but is outperformed by BIC~\cite{BIC} and WA~\cite{mainatining} on ImageNet-1000 with incremental step size 100. Note that training a image classification model for $1,000$ classes on ImageNet-1000 is a challenging task even outside the continual learning context and BIC is originally proposed for large scale continual learning. In addition, our method still achieves better results compared with ICARL~\cite{ICARL} and EEIL~\cite{EEIL}, which are both effective offline continual learning methods. It is worth noting that our method is the first to report results for continual learning on ImageNet-1000 in online scenario. 

\subsection{Results on CORE50}
\label{subsec: results on core50}

 \vspace{-0.1cm}
\subsection{Ablation Study}
\vspace{-0.1cm}
We also conduct ablation study under current protocol~\cite{ICARL} to analyze the effectiveness of each component in our proposed method including candidates selection with prior incorporation (CS) and exemplar augmentation in feature space (EA). Specifically, we regard our method without CS and EA as the \textbf{Baseline} and compare it with \textbf{Baseline + CS}, \textbf{Baseline + EA} and \textbf{Baseline + CS + EA}. We use CIFAR-100 with step size 10, 20, ImageNet-100 with step size 10 and ImageNet-1000 with step size 100 as examples. Results are shown in Figure~\ref{fig:ablation}. We observe consistent results with large improvement from \textbf{Baseline} to \textbf{Baseline + CS} and EA also helps to further improve the performance. In addition, we provide the confusion matrices as shown in Figure~\ref{fig:confusion } to analyze the results in detail. The \textbf{Baseline} tends to predict new classes more frequently and some improvement can be made with the help by EA. The CS is shown to be more effective to correct the prediction bias than EA and our method is able to treat new classes and old classes more fairly by combining both CS and EA. 
% \vspace{+0.3cm}
\subsection{Analysis of Storage Consumption}
% \vspace{+0.2cm}
\label{exp:Analysis of Weights Bias, Memory}
In this section, we implement additional experiments to show the advantages of our proposed method in online scenario including the analysis of norms of weight vectors in classifier and the comparisons of storage consumption.

\textbf{Norms of weight vectors: }One of the main reasons for catastrophic forgetting is the weights in trained model’s FC layer are heavily biased towards new classes, which is already discussed in offline mode~\cite{BIC,mainatining} but lacks sufficient study in online scenario. In addition, as introduced in Section~\ref{introduction}, our proposed method works under the observation that the weight bias problem is significantly alleviated in online scenario. Therefore, we provide analysis for the impact on biased weights in online and offline scenarios by (1) varying incremental step size and (2) applying exemplar set (Exp). For generality, we consider \textbf{CN} and \textbf{CN + Exp} as two baseline methods using regular cross entropy for continual learning without and with exemplars, respectively. We use CIFAR-100 with step size 5, 10 and 20 for experiments under protocol~\cite{ICARL}. We train 70 epochs in offline mode as in~\cite{ICARL,EEIL} and 1 epoch in online scenario for each learning step. Results are shown in Figure~\ref{fig:weightnorm}. Each dot corresponds to the norm of the weight vectors in FC layer for each class. For better visualization, we fit the dots using linear least square to show the trend of each method when new classes are added sequentially. 

We observe that the weight bias problem is getting more severe when the number of incremental steps increases, especially in offline case since we repeatedly update model using only new class data. The overall performance in online scenario is much better than offline as each data is used only once for training. 

Next, we show that using exemplars is effective to correct biased weights in both online and offline scenario as indicated by \textbf{CN+EXP} compared to \textbf{CN}. We additionally compare baseline methods with our methods \textbf{Ours} (freezing parameters in FC layer for all learned classes) and applying Weight Aligning~\cite{mainatining} denoted as \textbf{WA} for bias correction. The performance of using exemplars in online scenario is even better than applying WA in offline case and our proposed strategy further alleviate this problem. Both analysis explain the larger gains we achieved for smaller step size on CIFAR-100 as discussed in Section~\ref{exp:offlinecifarimagenet}. The comparison between online and offline results also show the potential to address catastrophic forgetting in online scenario with the benefit of reduced weight bias problem.  


\begin{figure}[t]
\begin{minipage}[t]{0.47\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/norms_new1.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(a)}
\end{minipage}
\hspace{2ex}
\begin{minipage}[t]{0.47\linewidth}
    \centering
    \includegraphics[width=4.cm,height=3.5cm]{exp_new/norms_new2.png}
    \parbox{15.5cm}{\small \hspace{2.cm}(b)}
\end{minipage}
\begin{center}  %\vspace{-0.2cm}
  \caption{\textbf{Norms of the weight vectors on CIFAR-100} for (a) the impact of different step size 5, 10, and 20. (b) Impact of different approaches using step size 5. The solid line is obtained by linear least square to show the trend for each case. More results can be found in supplementary material.}
  \vspace{-.9cm}
  \label{fig:weightnorm}
\end{center}
\end{figure}


\textbf{Storage consumption: } Storage requirement poses significant constrains for continual learning in online mode. If we can store all data seen so far without considering storage requirement in real world scenario, then we can easily update the model using all available data. Therefore, we compare the storage consumption of our method with existing approaches to show the significant reduction in storage requirement. Let $S$ denote the image size, $C$ denote the number of total classes seen so far, $Q$ refers to the number of data stored in exemplar set for each class and $D$ denotes the dimension of extracted feature embedding. (1) For methods using exemplar set for replay~\cite{prabhu2020gdumb_online,aljundi_mir,NEURIPS2019_e562cd9c_GSS, GEM, A-GEM,chaudhry2019_TINYER,chaudhry2020using_HAL}, the storage requirement for storing data in exemplar set is $O(3\times S^2 \times Q \times C)$. (2) For methods using both exemplar set and knowledge distillation~\cite{ICARL,EEIL,BIC,mainatining,ILIO}, the total storage is $O(3\times S^2 \times Q \times C + Q \times C^2)$ with an additional part to store output logits for distillation. (3) For methods which store statistics of old classes and conduct pseudo rehearsal~\cite{fearnet,cgan}, the total cost is $O(D^2 \times C)$ (4) For our method that store feature embeddings as exemplars, the total storage is $O(D \times C \times Q)$. Therefore, as $Q\ll D < 3\times S^2$, our method requires the least storage while still achieving the best performance.



